Quasi steady state approximation of the small clusters in Becker-D\"oring equations leads to boundary conditions in the Lifshitz-Slyozov limit

This papers addresses the connection between two classical models of phase transition phenomena describing different stages of the growth of clusters. The Becker-D\"oring model (BD) describes discrete-sized clusters through an infinite set of ordinary differential equations. The Lifshitz-Slyozov equation (LS) is a transport partial differential equation on the continuous half-line $x\in (0,+\infty)$. We introduce a scaling parameter $\varepsilon>0$, which accounts for the grid size of the state space in the BD model, and recover the LS model in the limit $\varepsilon\to 0$. The connection has been already proven in the context of outgoing characteristic at the boundary $x=0$ for the LS model, when small clusters tend to shrink. The main novelty of this work resides in a new estimate on the growth of small clusters, which behave at a fast time scale. Through a rigorous quasi steady state approximation, we derive boundary conditions for the incoming characteristic case, when small clusters tend to grow.

==> macros.tex <==
% Mise en page
% \hoffset = 0pt % + 1in = 72.27 pt
% \voffset = 0pt % + 1in = 72.27 pt
% \oddsidemargin = 20pt
% \evensidemargin = 20pt
% \topmargin = 0pt
% \headheight = 12pt
% \headsep = 20pt
% \textheight = 586pt
% \textwidth = 412,46002pt
% \footskip = 32pt
% \marginparwidth = 62pt
% \marginparsep = 20pt
% \marginparpush = 5pt
% \columnsep = 30pt
% \columnseprule = 0.0pt
% 
% \hfuzz=1pt

% Quelques packages

\usepackage[T1]{fontenc}
\usepackage{ae,aecompl}
% \usepackage[foot]{amsaddr}
\usepackage{amsfonts,amssymb,mathtools}
\usepackage{color}
%\usepackage{chemarr}
\usepackage{enumitem,cite}
% 
\setenumerate{label=\arabic*.,itemsep=3pt,topsep=3pt}

%%%% hyperref

%\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}


%%% theorem

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{hyp}{Assumption}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\theoremstyle{remark}
\newtheorem{remark}{Remark}

%%% mathstyle

\def\Ab{\mathbb A}
\def\Bb{\mathbb B}
\def\Cb{\mathbb C}
\def\Db{\mathbb D}
\def\Eb{\mathbb E}
\def\Fb{\mathbb F}
\def\Gb{\mathbb G}
\def\Hb{\mathbb H}
\def\Ib{\mathbb I}
\def\Jb{\mathbb J}
\def\Kb{\mathbb K}
\def\Lb{\mathbb L}
\def\Mb{\mathbb M}
\def\Nb{\mathbb N}
\def\Ob{\mathbb O}
\def\Pb{\mathbb P}
\def\Qb{\mathbb Q}
\def\Rb{\mathbb R}
\def\Sb{\mathbb S}
\def\Tb{\mathbb T}
\def\Ub{\mathbb U}
\def\Vb{\mathbb V}
\def\Wb{\mathbb W}
\def\Xb{\mathbb X}
\def\Yb{\mathbb Y}
\def\Zb{\mathbb Z}


\def\Ac{\mathcal A}
\def\Bc{\mathcal B}
\def\Cc{\mathcal C}
\def\Dc{\mathcal D}
\def\Ec{\mathcal E}
\def\Fc{\mathcal F}
\def\Gc{\mathcal G}
\def\Hc{\mathcal H}
\def\Ic{\mathcal I}
\def\Jc{\mathcal J}
\def\Kc{\mathcal K}
\def\Lc{\mathcal L}
\def\Mc{\mathcal M}
\def\Nc{\mathcal N}
\def\Oc{\mathcal O}
\def\Pc{\mathcal P}
\def\Qc{\mathcal Q}
\def\Rc{\mathcal R}
\def\Sc{\mathcal S}
\def\Tc{\mathcal T}
\def\Uc{\mathcal U}
\def\Vc{\mathcal V}
\def\Wc{\mathcal W}
\def\Xc{\mathcal X}
\def\Yc{\mathcal Y}
\def\Zc{\mathcal Z}

% \def\B
% \def\C
% \def\D
% \def\E
% \def\F
% \def\G
% \def\H
% \def\I
% \def\J
% \def\K
% \def\L
% \def\M
% \def\N
% \def\O
% \def\P
% \def\Q
% \def\R
% \def\S
% \def\T
% \def\U
% \def\V
% \def\W
% \def\X
% \def\Y
% \def\Z

%%% Greek

% List of greek letter and variant at http://www.combinatorics.net/weblib/a.2/a2.html

\def\veps{\varepsilon}
\def\vtheta{\vartheta}
\def\vkappa{\varkappa}
\def\vpi{varpi}
\def\vrho{\varrho}
\def\vsigma{\varsigma}
\def\vphi{\varphi}

%%% Norm & Scalar product, etc

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\Abs}[1]{\left\lvert #1 \right\rvert}

\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\Norm}[1]{\left\lVert #1 \right\rVert}

\newcommand{\sprod}[2]{( #1, #2 )}
\newcommand{\Sprod}[2]{\left( #1, #2 \right)}

\newcommand{\brak}[2]{\langle #1 , #2 \rangle}
\newcommand{\Brak}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\Enbrace}[1]{\left\{ #1 \right\}}

\def\lb{\langle}
\def\rb{\rangle}

%%% Special functions

\newcommand{\indic}[1]{\mathbf{1}_{#1}}
\newcommand{\Xindic}[1]{\chi_{#1}}


\newcommand{\prob}[1]{\mathbb{P}\big{\{}#1\big{\}}}
%\newcommand{\esp}[1]{\mathbb{E}\big{[}#1\big{]}}
\newcommand{\esp}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\espin}[2]{\mathbb{E}_{#1}\big{[}#2\big{]}}
\newcommand{\ind}[1]{\mathbf{1}_{\{ #1 \}}}


%%% Others

\def\ds{\displaystyle}
\def\Card{\operatorname{Card}}			% Cardinal d'un ensemble
\newcommand{\supp}{\mathrm{supp}}

\def\Id{\mathrm{Id}}
\def\ie{{\it i.e.}}

\def\as{{\it a.s.}}

